Towards the $p=3$ Kervaire Invariant Problem: The $E_2$-page for the homotopy fixed points spectral sequence computing $\pi_*({E_6}^{hC_9})$

Hill, Hopkins, and Ravenel suggest that the last remaining Kervaire invariant problem, the case of $p=3$, can be solved by computing the homotopy fixed points spectral sequence for $\pi_* E_6^{hC_9}$. We prove a detection theorem for this case and use a conjectural form of the $C_9$-action on $E_6$ to compute the $E_2$ page of this spectral sequence away from homological degree zero.

==> preamble/rs-extras2.tex <==
\newcommand{\rstitle}{}
\newcommand{\rsdate}{}
\newcommand{\rspaperauthor}{}
\newcommand{\rspapertitle}{}
\newcommand{\rspaper}{}
\newcommand{\rsperson}{}
\newcommand{\rsspeaker}{}
\newcommand{\rskeywords}{}
\newcommand{\rsevent}{}

\renewcommand{\title}[1]{\renewcommand{\rstitle}{#1}}
\renewcommand{\date}[1]{\renewcommand{\rsdate}{#1}}
\newcommand{\paper}[1]{\renewcommand{\rspaper}{#1}}
\newcommand{\person}[1]{\renewcommand{\rsperson}{#1}}
\newcommand{\speaker}[1]{\renewcommand{\rsspeaker}{#1}}
\renewcommand{\keywords}[1]{\renewcommand{\rskeywords}{#1}}
\newcommand{\event}[1]{\renewcommand{\rsevent}{#1}}


\renewcommand{\maketitle}{
\ifthenelse{\equal\rsspeaker{}}{
{\setstretch{1}
\begin{mdframed}[linecolor=black!50,backgroundcolor=black!2]
{\large \rstitle}
\end{mdframed}
%{\parskip=-10pt {\scalefont{1.2}\ding{43}}\ \ {\large \rstitle} \par\hrulefill\par}
%{\parskip=-10pt \ {\large \rstitle} \par\hrulefill\par}

{\parskip=2pt\hfill\parbox{0.7\linewidth}{%make indented box
	\begin{mdframed}[linecolor=white,backgroundcolor=black!3]
    {\parskip=-1pt\hangindent=10pt\scalefont{0.8}
    \ifthenelse{\equal\rsdate{}}{}
        {\par \hangindent=10pt{\bf Date:} \rsdate}
    \ifthenelse{\equal\rsperson{}}{}
        {\par \hangindent=10pt{{\bf Person:} \rsperson}}
    \ifthenelse{\equal\rspaper{}}{}
        {\par \hangindent=10pt{{\bf Paper discussed:} \rspaper}}
    \ifthenelse{\equal\rskeywords{}}{}
        {\par \hangindent=10pt{\bf Keywords:} \rskeywords}
	\par
    }\end{mdframed}
}}\hfill \vspace{10pt}}
}{
{\parskip=-10pt \scalefont{1.2}{\sc\Large \rstitle} \par\hrulefill\par}%
{\parskip=0pt
	\begin{minipage}[t]{0.22\linewidth}
	{\scalefont{0.8}Notes from a talk by:}
	\end{minipage}
	\begin{minipage}[t]{0.80\linewidth}
	{\ifthenelse{\equal\rsspeaker{}}{}
        {\par {\large\sc \rsspeaker}\vspace{2pt}}
    {\scalefont{0.8}
    \ifthenelse{\equal\rsevent{}}{}
        {\par{\it \rsevent}}
    \ifthenelse{\equal\rsdate{}}{}
        {\par{\it \rsdate}}
    \ifthenelse{\equal\rspaper{}}{}
        {\par {\color{mgray}{Paper discussed:} \rspaper}}
    \ifthenelse{\equal\rskeywords{}}{}
        {\par {\color{mgray}{Keywords:} \rskeywords}}
	\par
    }}
	\end{minipage}
	\vspace{10pt}
}%non-title 
}%no speaker
}%maketitle

%Copied from https://tex.stackexchange.com/questions/30720/footnote-without-a-marker
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

